Deep End-to-End Alignment and Refinement for Time-of-Flight RGB-D Module

Recently, it is increasingly popular to equip mobile RGB cameras with Time-of-Flight (ToF) sensors for active depth sensing. However, for off-the-shelf ToF sensors, one must tackle two problems in order to obtain high-quality depth with respect to the RGB camera, namely 1) online calibration and alignment; and 2) complicated error correction for ToF depth sensing. In this work, we propose a framework for jointly alignment and refinement via deep learning. First, a cross-modal optical flow between the RGB image and the ToF amplitude image is estimated for alignment. The aligned depth is then refined via an improved kernel predicting network that performs kernel normalization and applies the bias prior to the dynamic convolution. To enrich our data for end-to-end training, we have also synthesized a dataset using tools from computer graphics. Experimental results demonstrate the effectiveness of our approach, achieving state-of-the-art for ToF refinement.

==> arch_nouse.tex <==
We used the FlowNetC for the cross-modal optical flow estimation task. 
Therefore we refer the readers to \cite{dosovitskiy2015flownet} for its detailed architecture. 
Since FlowNetC takes two three-channel images as inputs, we repeat the one-channel ToF amplitude for three times before feeding it to FlowNetC.
The detailed architectures of the flow fusion network and the backbone of the depth refinement networks are provided in Table\,\ref{tab:flow_fuse} and Table\,\ref{tab:depth_net}, respectively.
Both of these networks are U-Nets with skip connections.
%
\begin{table}[htbp]\fontsize{7.5pt}{7.5pt}\selectfont
  \centering
  \renewcommand{\tabcolsep}{3.2pt}
  \renewcommand{\arraystretch}{1}
   \begin{tabular}{|m{24pt}<{\centering}|m{5pt}<{\centering}m{5pt}<{\centering}m{30pt}<{\centering}|m{5pt}<{\centering}m{5pt}<{\centering}|m{75pt}<{\centering}|}
    %\begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
   \textbf{Layer} & \textbf{K} & \textbf{S} & \textbf{Channels} & \textbf{I} & \textbf{O} & \textbf{Input Channels} \bigstrut\\
    \hline
    conv0 & 3$\times$3   & 1     & 4/64  & 512$\times$384 & 512$\times$384 & flow\_base,\\flow\_pose \bigstrut[t]\\
    conv1 & 3$\times$3   & 2     & 64/64 & 512$\times$384 & 256$\times$192 & conv0 \\
    conv1\_1 & 3$\times$3   & 1     & 64/128 & 256$\times$192 & 256$\times$192 & conv1 \\
    conv2 & 3$\times$3   & 2     & 128/128 & 256$\times$192 & 128$\times$96 & conv1\_1 \\
    conv2\_1 & 3$\times$3   & 1     & 128/128 & 128$\times$96 & 128$\times$96 & conv2 \bigstrut[b]\\
    \hline
    flow2 & 3$\times$3   & 1     & 128/2 & 128$\times$96 & 128$\times$96 & conv2\_1 \bigstrut\\
    \hline
    upconv1 & 4$\times$4   & 2     & 128/64 & 128$\times$96 & 256$\times$192 & conv2\_1 \bigstrut[t]\\
    rconv1 & 3$\times$3   & 1     & 162/32 & 256$\times$192 & 256$\times$192 & upconv1,flow2,conv1\_1 \bigstrut[b]\\
    \hline
    flow1 & 3$\times$3   & 1     & 32/2  & 256$\times$192 & 256$\times$192 & rconv1 \bigstrut\\
    \hline
    upconv0 & 4$\times$4   & 2     & 32/16 & 256$\times$192 & 512$\times$384 & rconv1 \bigstrut[t]\\
    rconv0 & 3$\times$3   & 1     & 82/16 & 512$\times$384 & 512$\times$384 & upconv0，flow1,conv0 \bigstrut[b]\\
    \hline
    flow2 & 3$\times$3   & 1     & 16/2  & 512$\times$384 & 512$\times$384 & rconv0 \bigstrut\\
    \hline
    \end{tabular}%
    \caption{Architecture of the optical flow fusion network.}
  \label{tab:flow_fuse}%
\end{table}%

\begin{table}[htbp]\fontsize{7.5pt}{7.5pt}\selectfont
  \centering
   \renewcommand{\tabcolsep}{3.2pt}
  \renewcommand{\arraystretch}{1}
  
    \begin{tabular}{|l|lrl|ll|l|}
    \hline
    Name  & Kenel & \multicolumn{1}{l}{Str.} & Ch I/O & In Res & Out Res & Inputs \bigstrut\\
    \hline
    conv0 & 3$\times$3   & 1     & 5/64  & 512$\times$384 & 512$\times$384 & f\_depth, bl\_dpeth, RGB \bigstrut[t]\\
    conv1 & 3$\times$3   & 2     & 64/128 & 512$\times$384 & 256$\times$192 & conv0 \\
    conv1\_1 & 3$\times$3   & 1     & 128/256 & 256$\times$192 & 256$\times$192 & conv1 \\
    conv2 & 3$\times$3   & 2     & 256/256 & 256$\times$192 & 128$\times$96 & conv1\_1 \\
    conv2\_1 & 3$\times$3   & 1     & 256/256 & 128$\times$96 & 128$\times$96 & conv2 \bigstrut[b]\\
    \hline
    depth2 & 3$\times$3   & 1     & 256/1 & 128$\times$96 & 128$\times$96 & conv2\_1 \bigstrut\\
    \hline
    upconv1 & 4$\times$4   & 2     & 256/64 & 128$\times$96 & 256$\times$192 & conv2\_1 \bigstrut[t]\\
    rconv1 & 3$\times$3   & 1     & 321/64 & 256$\times$192 & 256$\times$192 & upconv1,depth2,conv1\_1 \bigstrut[b]\\
    \hline
    depth1 & 3$\times$3   & 1     & 64/1  & 256$\times$192 & 256$\times$192 & rconv1 \bigstrut\\
    \hline
    upconv0 & 4$\times$4   & 2     & 64/32 & 256$\times$192 & 512$\times$384 & rconv1 \bigstrut[t]\\
    rconv0 & 3$\times$3   & 1     & 97/32 & 512$\times$384 & 512$\times$384 & upconv0,depth1,conv0 \bigstrut[b]\\
    \hline
    depth0 & 3$\times$3   & 1     & 32/1  & 512$\times$384 & 512$\times$384 & rconv0 \bigstrut\\
    \hline
    \end{tabular}%
    \vspace{3pt}
    \caption{Net Architecture of depth refinement network. Detailed architecture of the proposed \emph{DispFulNet}. The layer {\tt corr} is the correlation layer of \cite{mayer16} with maximum displacement 40, while layers with prefix {\tt pr\_} are convolution layers output disparity images at multiple scales. {\bf K} means kernel size, {\bf S} means stride, and {\bf Channels} is the number of input and output channels. {\bf I} and {\bf O} are the input and output downsampling factor relative to the input. The symbol {\tt +} means concatenation.}
  \label{tab:depth_net}%
\end{table}%

